Universal Link Predictor By In-Context Learning on Graphs

Link prediction is a crucial task in graph machine learning, where the goal is to infer missing or future links within a graph. Traditional approaches leverage heuristic methods based on widely observed connectivity patterns, offering broad applicability and generalizability without the need for model training. Despite their utility, these methods are limited by their reliance on human-derived heuristics and lack the adaptability of data-driven approaches. Conversely, parametric link predictors excel in automatically learning the connectivity patterns from data and achieving state-of-the-art but fail short to directly transfer across different graphs. Instead, it requires the cost of extensive training and hyperparameter optimization to adapt to the target graph. In this work, we introduce the Universal Link Predictor (UniLP), a novel model that combines the generalizability of heuristic approaches with the pattern learning capabilities of parametric models. UniLP is designed to autonomously identify connectivity patterns across diverse graphs, ready for immediate application to any unseen graph dataset without targeted training. We address the challenge of conflicting connectivity patterns-arising from the unique distributions of different graphs-through the implementation of In-context Learning (ICL). This approach allows UniLP to dynamically adjust to various target graphs based on contextual demonstrations, thereby avoiding negative transfer. Through rigorous experimentation, we demonstrate UniLP's effectiveness in adapting to new, unseen graphs at test time, showcasing its ability to perform comparably or even outperform parametric models that have been finetuned for specific datasets. Our findings highlight UniLP's potential to set a new standard in link prediction, combining the strengths of heuristic and parametric methods in a single, versatile framework.

==> body/experiment.tex <==
\section{Experiments}
In this section, we conduct extensive experiments to assess the performance of \our on new unseen datasets.

% \begin{table}[h]
%     \centering
%     \caption{The pretrain and test datasets.}\label{tab:stats}
%     \resizebox{\linewidth}{!}{%
%     % insert
%     \begin{tabular}{lcc|ccc}
%     \toprule
%         \textbf{Dataset} & \textbf{Pretrain} & \textbf{Test} & \textbf{\# Nodes} & \textbf{\# Edges} & \textbf{Avg. node deg.}\\
%     \midrule\rowcolor{Gray}
%     \multicolumn{6}{c}{\textbf{Biology}} \\
%     Ecoli &\Checkmark & - & 1805 & 29320 & 16.24\\
%     Yeast &\Checkmark & - & 2375 & 23386 & 9.85\\
%     Celegans &- & \Checkmark & 297 & 4296 & 14.46\\
%     \midrule
%     \rowcolor{Gray}
%     \multicolumn{6}{c}{\textbf{Transport}} \\
%     Power &\Checkmark & - & 4941 & 13188 & 2.67\\
%     USAir &- & \Checkmark & 332 & 4252 & 12.81\\
%     \midrule
%     \rowcolor{Gray}
%     \multicolumn{6}{c}{\textbf{Web}} \\
%     PolBlogs &\Checkmark & - & 1490 & 19025 & 12.77\\
%     Router &\Checkmark & - & 5022 & 12516 & 2.49\\
%     PB &- & \Checkmark & 1222 & 33428 & 27.36\\
%     \midrule
%     \rowcolor{Gray}
%     \multicolumn{6}{c}{\textbf{Collaboration}} \\
%     Physics &\Checkmark & - & 34493 & 495924 & 14.38\\
%     CS &- & \Checkmark & 18333 & 163788 & 8.93\\
%     NS &- & \Checkmark & 1589 & 5484 & 3.45\\
%     \midrule
%     \rowcolor{Gray}
%     \multicolumn{6}{c}{\textbf{Citation}} \\
%     Pubmed &\Checkmark & - & 19717 & 88648 & 4.5\\
%     Citeseer &\Checkmark & - & 3327 & 9104 & 2.74\\
%     Cora &- & \Checkmark & 2708 & 10556 & 3.9\\
%     \midrule
%     \rowcolor{Gray}
%     \multicolumn{6}{c}{\textbf{Social}} \\
%     Twitch &\Checkmark & - & 34118 & 429113 & 12.58\\
%     Github &\Checkmark & - & 37700 & 289003 & 7.67\\
%     Facebook &- & \Checkmark & 22470 & 171002 & 7.61\\
%     \bottomrule
%     \end{tabular}
%     % until
% }
% \end{table}

\subsection{Experimental setup}
\mao{If the space is not enough, I think we can remove this section title}
\paragraph{Benchmark datasets.} The foundation for our model's training is a collection of graph datasets spanning a variety of domains. Following~\cite{mao_revisiting_2023}, we have carefully selected \mao{diverse} graph data from fields such as biology~\cite{von_mering_comparative_2002,zhang_beyond_2018,watts_collective_1998}, transport~\cite{watts_collective_1998,batagelj_pajek_2006}, web~\cite{ackland_mapping_2005,spring_measuring_2002,adamic_political_2005}, academia collaboration~\cite{shchur_pitfalls_2019,newman_finding_2006}, citation~\cite{yang_revisiting_2016}, and social networks~\cite{rozemberczki_multi-scale_2021}. This diverse selection ensures that we can pretrain and evaluate the LP model based on a wide array of connectivity patterns. The details of the curated graph datasets can be found in Table~\ref{tab:stats} in Appendix.

% Moreover, the datasets vary not only in domain but also in type and scale. They include both weighted and unweighted graphs, as well as directed and undirected structures. The size of these graphs ranges significantly, with the number of nodes varying from $10^2$ to $10^6$ and the number of edges ranging from $10^4$ to $10^6$. The comprehensive details of these graph datasets are shown in Table~\ref{tab:stats}.

\paragraph{Baseline Methods.} We compare \our with both heuristic and GNN-based parametric link predictors. Heuristic methods include Common Neighbor (CN)~\cite{liben-nowell_link_2003}, Adamic-Adar index (AA)~\cite{adamic_friends_2003}, Resource Allocation (RA)~\cite{zhou_predicting_2009}, Preferential Attachment (PA)~\cite{barabasi_emergence_1999}, Shortest-Path (SP), and Katz index (Katz)~\cite{katz_new_1953}. GNN-based methods include GAE~\cite{kipf_variational_2016}, SEAL~\cite{zhang_link_2018}, ELPH~\cite{chamberlain_graph_2022}, NCNC~\cite{wang_neural_2023}, and MPLP~\cite{dong_pure_2023}.  For GAE and NCNC, which require initial node features, we use a $32$-dimensional all-one vector. All other methods can handle non-attributed graphs directly.

\paragraph{Evaluation of \our.} To evaluate \our's effectiveness on unseen datasets, we divide our graph data into non-overlapping pretrain and testing sets (see Table~\ref{tab:stats}) and pretrain one single model on the combined pretrain datasets. During pretraining, we dynamically sample $40$ positive and negative links as in-context links $S^+ \cup S^-$ for each query link from the corresponding pretrain dataset. For evaluation, each test dataset is split into 70\%/10\%/20\% for training/validation/testing. The training set here forms the observed links $E^o$, while validation and test sets represent unobserved links $E^u$. During the inference, we sample $200$ positive and negative links as in-context links per test dataset. We report Hits@50~\cite{hu_open_2021} as the evaluation metric for LP. More details about the pretraining of \our can be found in Appendix~\ref{app:pretrain}. 
\mao{I think since we only pre-train on one dataset we need to emphasize which dataset we utilize for pre-train and how it divergers from other dataset. This is an important experimental setting}

\paragraph{Evaluation of Baselines.} Baseline models follow similar evaluation procedures, with adaptations for transfer learning capabilities. We employ two settings: (1) \textbf{Pretrain Only}, where models are trained on combined pretrain datasets \mao{Why here is combined pretrain datasets} and then tested on each test dataset, and (2) \textbf{Pretrain \& Finetune}, where after pretraining, models are additionally finetuned on each test dataset with $200$ sampled positive and negative links for training.

\subsection{Primary results}

\begin{table*}[h]
    \centering
    \caption{Link prediction results on test datasets evaluated by Hits@50. The format is average score ± standard deviation. The top three models are colored by \textbf{\textcolor{red}{First}}, \textbf{\textcolor{blue}{Second}}, \textbf{\textcolor{violet}{Third}}.}\label{tab:real}
    \resizebox{\textwidth}{!}{%
    % insert
    \begin{tabular}{lcccccccc}
    \toprule
    % \rowcolor{Gray}
            &\multicolumn{1}{c}{Biology}&\multicolumn{1}{c}{Transport}&\multicolumn{1}{c}{Web}&\multicolumn{2}{c}{Collaboration}&\multicolumn{1}{c}{Citation}&\multicolumn{1}{c}{Social}\\ \cmidrule(r{0.5em}){2-2} \cmidrule(r{0.5em}){3-3} \cmidrule(r{0.5em}){4-4} \cmidrule(r{0.5em}){5-6} \cmidrule(r{0.5em}){7-7} \cmidrule(r{0.5em}){8-8} 
            
        & \textbf{C.ele} & \textbf{USAir} & \textbf{PB} & \textbf{NS} & \textbf{CS} & \textbf{Cora} & \textbf{Facebook} & \textbf{Ave. Rank}\\
    
        \midrule
        \rowcolor{Gray}
        \multicolumn{9}{c}{Heuristics} \\
        \textbf{CN} & $46.88 {\scriptstyle \pm 12.28}$ & $82.75 {\scriptstyle \pm 1.54}$ & $41.15 {\scriptstyle \pm 3.77}$ & $74.03 {\scriptstyle \pm 1.59}$ & $56.84 {\scriptstyle \pm 15.56}$ & $33.85 {\scriptstyle \pm 0.93}$ & $58.70 {\scriptstyle \pm 0.35}$ & 11.00 \\
    \textbf{AA} & $61.07 {\scriptstyle \pm 5.16}$ & \thirdt{86.96}{2.24} & $44.12 {\scriptstyle \pm 3.36}$ & $74.03 {\scriptstyle \pm 1.59}$ & \thirdt{68.22}{1.08} & $33.85 {\scriptstyle \pm 0.93}$ & \secondt{67.80}{2.12} & 5.71 \\
    \textbf{RA} & $62.80 {\scriptstyle \pm 4.84}$ & \secondt{87.27}{1.89} & $43.72 {\scriptstyle \pm 2.86}$ & $74.03 {\scriptstyle \pm 1.59}$ & $68.21 {\scriptstyle \pm 1.08}$ & $33.85 {\scriptstyle \pm 0.93}$ & \firstt{68.84}{2.03} & 5.57 \\
    \textbf{PA} & $43.85 {\scriptstyle \pm 4.12}$ & $77.69 {\scriptstyle \pm 2.29}$ & $28.93 {\scriptstyle \pm 1.91}$ & $35.35 {\scriptstyle \pm 3.01}$ & $6.49 {\scriptstyle \pm 0.61}$ & $22.09 {\scriptstyle \pm 1.52}$ & $12.95 {\scriptstyle \pm 0.63}$ & 13.71 \\
    \textbf{SP} & $0.00 {\scriptstyle \pm 0.00}$ & $0.00 {\scriptstyle \pm 0.00}$ & $0.00 {\scriptstyle \pm 0.00}$ & $80.00 {\scriptstyle \pm 1.11}$ & $41.34 {\scriptstyle \pm 35.58}$ & $52.97 {\scriptstyle \pm 1.53}$ & $0.00 {\scriptstyle \pm 0.00}$ & 13.14 \\
    \textbf{Katz} & $58.86 {\scriptstyle \pm 6.48}$ & $84.64 {\scriptstyle \pm 1.86}$ & $44.36 {\scriptstyle \pm 3.65}$ & $78.96 {\scriptstyle \pm 1.35}$ & $66.32 {\scriptstyle \pm 5.59}$ & $52.97 {\scriptstyle \pm 1.53}$ & $60.79 {\scriptstyle \pm 0.60}$ & 6.86 \\
    
        \midrule
        \rowcolor{Gray}
        \multicolumn{9}{c}{Pretrain Only} \\
        \textbf{SEAL} & $61.28 {\scriptstyle \pm 3.76}$ & $86.00 {\scriptstyle \pm 1.56}$ & $45.44 {\scriptstyle \pm 2.68}$ & $84.07 {\scriptstyle \pm 1.96}$ & $62.82 {\scriptstyle \pm 1.62}$ & $56.21 {\scriptstyle \pm 2.24}$ & $54.57 {\scriptstyle \pm 1.48}$ & 5.57 \\
    \textbf{GAE} & $44.71 {\scriptstyle \pm 3.39}$ & $76.12 {\scriptstyle \pm 2.27}$ & $27.56 {\scriptstyle \pm 2.34}$ & $15.20 {\scriptstyle \pm 2.14}$ & $5.08 {\scriptstyle \pm 0.48}$ & $24.22 {\scriptstyle \pm 1.53}$ & $6.65 {\scriptstyle \pm 0.57}$ & 14.14 \\
    \textbf{ELPH} & $59.23 {\scriptstyle \pm 4.50}$ & $84.42 {\scriptstyle \pm 2.22}$ & $43.69 {\scriptstyle \pm 2.90}$ & $84.27 {\scriptstyle \pm 1.43}$ & \secondt{70.69}{3.63} & $56.91 {\scriptstyle \pm 1.43}$ & $61.80 {\scriptstyle \pm 2.46}$ & 5.57 \\
    \textbf{NCNC} & $48.07 {\scriptstyle \pm 4.79}$ & $75.44 {\scriptstyle \pm 4.22}$ & $25.66 {\scriptstyle \pm 1.42}$ & $80.07 {\scriptstyle \pm 1.43}$ & $34.27 {\scriptstyle \pm 2.28}$ & $52.51 {\scriptstyle \pm 2.54}$ & $19.28 {\scriptstyle \pm 1.58}$ & 11.57 \\
    \textbf{MPLP} & $56.74 {\scriptstyle \pm 5.31}$ & $82.94 {\scriptstyle \pm 2.30}$ & \thirdt{47.78}{2.55} & $80.33 {\scriptstyle \pm 1.54}$ & $24.26 {\scriptstyle \pm 1.28}$ & $46.71 {\scriptstyle \pm 2.25}$ & $48.06 {\scriptstyle \pm 2.09}$ & 8.86 \\
    
        \midrule
        \rowcolor{Gray}
        \multicolumn{9}{c}{Pretrain \& Finetune} \\
        \textbf{SEAL} & \thirdt{64.45}{4.14} & \firstt{88.49}{2.16} & $47.78 {\scriptstyle \pm 3.32}$ & $84.84 {\scriptstyle \pm 2.32}$ & $61.54 {\scriptstyle \pm 3.09}$ & \firstt{62.19}{3.27} & $58.70 {\scriptstyle \pm 2.78}$ & \secondts{3.14} \\
    \textbf{GAE} & $44.71 {\scriptstyle \pm 4.07}$ & $74.47 {\scriptstyle \pm 2.96}$ & $25.92 {\scriptstyle \pm 2.64}$ & $18.34 {\scriptstyle \pm 2.27}$ & $4.95 {\scriptstyle \pm 0.44}$ & $25.31 {\scriptstyle \pm 1.48}$ & $6.11 {\scriptstyle \pm 0.39}$ & 14.71 \\
    \textbf{ELPH} & $60.51 {\scriptstyle \pm 5.72}$ & $84.52 {\scriptstyle \pm 2.08}$ & $43.58 {\scriptstyle \pm 3.48}$ & \thirdt{86.08}{0.69} & \firstt{71.10}{3.48} & $57.18 {\scriptstyle \pm 1.89}$ & $63.31 {\scriptstyle \pm 3.63}$ & 4.71 \\
    \textbf{NCNC} & \secondt{64.45}{5.10} & $85.85 {\scriptstyle \pm 2.46}$ & $47.75 {\scriptstyle \pm 6.90}$ & \secondt{88.25}{2.25} & $58.75 {\scriptstyle \pm 5.74}$ & \secondt{60.00}{2.50} & $59.32 {\scriptstyle \pm 6.93}$ & \thirdts{3.71} \\
    \textbf{MPLP} & $62.56 {\scriptstyle \pm 4.79}$ & $85.08 {\scriptstyle \pm 1.54}$ & \secondt{48.01}{2.94} & $80.16 {\scriptstyle \pm 1.18}$ & $50.35 {\scriptstyle \pm 1.01}$ & $56.02 {\scriptstyle \pm 2.09}$ & $56.72 {\scriptstyle \pm 1.20}$ & 6.14 \\
    
        \midrule
        \rowcolor{Gray}
        \multicolumn{9}{c}{Ours} \\
        \textbf{UniLP} & \firstt{65.20}{4.40} & $85.98 {\scriptstyle \pm 2.00}$ & \firstt{48.14}{2.99} & \firstt{89.09}{2.05} & $64.59 {\scriptstyle \pm 2.65}$ & \thirdt{57.50}{2.40} & \thirdt{65.49}{2.05} & \firstts{1.86} \\
    \bottomrule
    \end{tabular}
    % until
}%\vspace{-8pt}
\end{table*}

Table~\ref{tab:real} presents the performance of \our on various unseen graph datasets. The results demonstrate that \our outperforms both traditional heuristic methods and standard GNN-based LP models that are pretrained without specific adaptation, showing significant improvements in 4 out of 7 the benchmark datasets. This performance enhancement suggests that tailoring the LP model to individual graphs can markedly increase its transfer learning capabilities.

\mao{Can we claim the finetuning is time consuming, and requires hyperparameter tuning}
Moreover, \our achieves comparable or even superior results to GNN-based LP models that undergo finetuning, \mao{Put the following on the front?} despite not being explicitly trained on the test data. This highlights the effectiveness of the ICL capability in \our, which allows the model to adapt seamlessly to specific graph datasets without the need for additional training. By leveraging in-context links provided during the inference phase, \our can dynamically adjust its knowledge of connectivity patterns, demonstrating its potential to deliver robust performance across a wide range of unseen graph datasets. In addition, the experimental results on the synthetic Triangular/Grid lattice graphs can be found in Table~\ref{tab:syn} in the Appendix.

\subsection{The inner mechanism of \our}
\begin{table*}[h]
    \centering
    \caption{Link prediction results on test datasets evaluated by Hits@50 under context perturbation. This table presents the outcomes of link prediction when the context, i.e., in-context links, is deliberately altered. The aim is to analyze how changes in the context influence the final prediction accuracy.}\label{tab:perturb}
    \resizebox{\textwidth}{!}{%
    % insert
    \begin{tabular}{lccccccc}
    \toprule
    % \rowcolor{Gray}
            &\multicolumn{1}{c}{Biology}&\multicolumn{1}{c}{Transport}&\multicolumn{1}{c}{Web}&\multicolumn{2}{c}{Collaboration}&\multicolumn{1}{c}{Citation}&\multicolumn{1}{c}{Social}\\ \cmidrule(r{0.5em}){2-2} \cmidrule(r{0.5em}){3-3} \cmidrule(r{0.5em}){4-4} \cmidrule(r{0.5em}){5-6} \cmidrule(r{0.5em}){7-7} \cmidrule(r{0.5em}){8-8} 
            
        & \textbf{C.ele} & \textbf{USAir} & \textbf{PB} & \textbf{NS} & \textbf{CS} & \textbf{Cora} & \textbf{Facebook}\\\midrule
    \textbf{UniLP-FlipLabel} & $0.61 {\scriptstyle \pm 0.27}$ & $15.81 {\scriptstyle \pm 13.17}$ & $0.03 {\scriptstyle \pm 0.03}$ & $27.97 {\scriptstyle \pm 4.29}$ & $0.60 {\scriptstyle \pm 0.23}$ & $2.03 {\scriptstyle \pm 0.55}$ & $0.32 {\scriptstyle \pm 0.15}$ \\
    \textbf{UniLP-RandomContext} & $52.89 {\scriptstyle \pm 5.90}$ & $81.91 {\scriptstyle \pm 2.14}$ & $47.47 {\scriptstyle \pm 3.05}$ & $85.60 {\scriptstyle \pm 1.23}$ & $47.80 {\scriptstyle \pm 6.48}$ & $37.62 {\scriptstyle \pm 5.64}$ & $22.17 {\scriptstyle \pm 6.55}$ \\ \midrule
    \textbf{UniLP} & $65.20 {\scriptstyle \pm 4.40}$ & $85.98 {\scriptstyle \pm 2.00}$ & $48.14 {\scriptstyle \pm 2.99}$ & $89.09 {\scriptstyle \pm 2.05}$ & $64.59 {\scriptstyle \pm 2.65}$ & $57.50 {\scriptstyle \pm 2.40}$ & $65.49 {\scriptstyle \pm 2.05}$ \\
    \bottomrule
    \end{tabular}
    % until
}%\vspace{-8pt}
\end{table*}
% This experiment examines how the quality of in-context links affects LP performance of \our. Since we consider each in-context link as a pair comprising an input and its corresponding label, we can conduct two types of perturbations on the in-context links: \textbf{FlipLabel}: we invert the labels of the in-context links, labeling previously positive links as negative and vice versa. \textbf{RandomContext}: Instead of selecting in-context links from the target graph, we randomly sample them from a graph generated using the Stochastic Block Model~\cite{holland_stochastic_1983}. 

% The outcomes, as shown in Table~\ref{tab:perturb}, reveal that flipping the labels of in-context links significantly degrades the model's performance, rendering it almost ineffective. This suggests that the accuracy of label information in in-context links is critical for enabling the ICL feature of \our. Such an adversarial perturbation can confuse the model regarding the underlying connectivity patterns.

We further explore the capability of our proposed model's ICL to facilitate skill learning~\cite{pan_what_2023,mao_data_2024}, enabling the model to acquire new skills not encountered during the pretraining phase, guided by ICL demonstrations. This investigation focuses on the model's performance sensitivity to corrupting in-context links, particularly when these links are presented with incorrect input-label associations. Given that each in-context link consists of an input and its corresponding label, we introduce two perturbation strategies to assess this sensitivity: \textbf{FlipLabel}: we invert the labels of the in-context links, labeling previously positive links as negative and vice versa. \textbf{RandomContext}: Instead of selecting in-context links from the target graph, we randomly sample them from a graph generated using the Stochastic Block Model~\cite{holland_stochastic_1983}. 

The outcomes, as shown in Table~\ref{tab:perturb}, reveal that flipping the labels of in-context links significantly degrades the model's performance, rendering it almost ineffective. This finding underscores the model's utilization of ICL for skill learning, specifically in learning new feature-label mappings within a given context~\cite{wei_larger_2023,min_rethinking_2022}. It highlights the pivotal role of accurate label information in in-context links for the model's effective adaptation to the target graph.

Furthermore, using randomly generated graphs as a source of in-context links also detrimentally affects performance, albeit to varying extents across different datasets. This implies the importance of choosing in-context links that genuinely represent the properties of the target graph. Interestingly, the less severe performance decline in some datasets may indicate their inherent community-based graph structures.

\begin{figure*}[h]
% \vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=\textwidth]{figure/more_context.png}}
\caption{Performance of \our with varying quantities of in-context links.}\label{fig:more_context}
\end{center}
% \vspace{-30pt}
\end{figure*}



% \mao{the following is by me}
% We then investigate the inner mechanism of the ICL ability of our proposed. 
% Following the ICL literature~\cite{pan2023context, mao2024data} in LLM, the ICL can be with two abilities, skill recognition and skill learning. Typically, The skill recognition ability recognizes the underlying skill of demonstrations and utilizes prior knowledge embedded in weights to solve the downstream task. In contrast, the skill learning ability can learn new skills, according to ICL demonstrations, unseen in the pre-training stage. 
% Typically, we examine whether the ICL on link prediction aligns with the skill recognition ability or the skill learning one via the performance sensitivity on corrupting in-context data with incorrect input-label mapping. If the LLM takes advantage of the skill learning ability more, the LLM can learn the corrupted in-context mapping, leading to performance degradation compared with the origin setting. In contrast, if the LLM follows the skill recognition ability more, the LLM should be robust to the correctness of
% the input-label mapping, since the skill recognition ability only implements the pre-training data generation function
% with correct input-label mapping. 
% we then conduct two corruptions on the in-context link examples following the literature~\cite{wei2023larger,min2022rethinking} in NLP. 
% \textbf{FlipLabel}: we flip the labels of the in-context link examples, labeling previously positive as negative and vice versa. 
% \textbf{RandomContext}: Instead of selecting in-context links from the target graph, we randomly sample them from a graph generated using the Stochastic Block Model~\cite{holland_stochastic_1983}. 
% Notably, FlipLabel is a much stronger permutation totally transforms the original feature-label mapping into the opposite one while the RandomContext may still illustrate certain alignment with the ground truth. 

% Experimental results, as shown in Table~\ref{tab:perturb}, reveal that flipping the labels of in-context link examples significantly degrades the model's performance, rendering it almost ineffective. This reveals that ICL implements the skill learning ability to learn the new feature-label mapping in context. 
% Similar observations can be found in RandomContext with a relatively smaller performance gap.


\subsection{Effectiveness of in-context links' size}
This experiment evaluates how varying the quantity of in-context links affects \our's performance during inference. We experiment with different numbers of in-context links, ranging from 10 to 400, sampled from each test graph \mao{What is sampled from each test graph means?}. These links are used as context for the model. Additionally, we utilize SEAL as the base model and assess its performance under finetuning (FT) and supervised training (SUP) from scratch with varying training sample sizes. For comparison, we also include results from training a SEAL model on the full set of target graph data (Full), as detailed in Figure~\ref{fig:more_context}.

The findings reveal a consistent improvement in \our's performance with an increasing number of in-context links. \mao{How about compare with other methods the relatively increasing speed.} This indicates that our method can more effectively capture the target graph's properties with additional context. Notably, on four of the test datasets, \our either matches or exceeds the performance of models trained end-to-end on the entire graph. This suggests that leveraging more pretrpretrain data can be advantageous for LP tasks when properly managed. Furthermore, despite both \our and the finetuned models being pretrained on the same datasets and using the same in-context links, \our occasionally outperforms its finetuned counterparts. This observation suggests that in some cases, utilizing ICL can be a more effective approach for adapting a pretrained model to a specific target dataset compared to finetuning. The trend on the rest of graphs can be found in Figure~\ref{fig:more_context_rest}.

\subsection{Visualization of the link representation}
We conduct a comparative visualization of link representations as learned by a Pretrained Only SEAL model and \our. This comparison is shown in Figure~\ref{fig:tsne}. The results indicate that a naively pretrained model tends to map link representations from various graph datasets into a close subspace, potentially leading to indistinguishable link representations across different graphs, even when these graphs exhibit conflicting connectivity patterns.
\begin{figure}[h]
    \centering
\begin{subfigure}[h]{0.5 \linewidth}
    \includegraphics[width=\linewidth]{figure/embedding_pretrain.png}
    % \caption{}   
    \vspace{-6mm}
    \subcaption{\label{fig:pretrain}}
    
\end{subfigure}%
% \hspace{5mm}
\begin{subfigure}[h]{0.5 \linewidth}
    \centering
    \includegraphics[width=\linewidth]{figure/embedding_icl.png}
    % \caption{}
    \vspace{-6mm}
    \subcaption{\label{fig:icl}}
    
\end{subfigure}
\vspace{-3mm}
\caption{Visualization of the link representation learned from (a) Pretrain Only SEAL; (b) \our. Different colors indicate different test datasets.}\label{fig:tsne}
\vspace{-4mm}
\end{figure}

In contrast, the link representations generated by \our, which are conditioned on the context of the target graph, demonstrate a distinct separation between different datasets. This separation is indicative of \our's effective ICL capability, which adeptly captures the subtle distributional differences across graphs. By adjusting the link representations based on the context provided by in-context links, \our can effectively address the challenge of conflicting connectivity patterns in diverse graph datasets.
% We further conduct additional experiments to evaluate the ICL ability of \our. (1) We select different sets of in-context links from each target graph to evaluate how the selection of the in-context links can affect the LP performance. We find that \our exhibits varying degrees of robustness across different datasets (Appendix~\ref{app:diverse}). (2) We use a varying ratio of positive-to-negative in-context links during the test time rather than a balanced set, and we find that in-context links comprising of only negative samples can perform as good as the balanced one on most of the datasets (Appendix~\ref{app:ratio}).
\vspace{-3mm}
\subsection{Additional experiments}
We carry out further experiments to investigate the ICL capabilities of \our: \textbf{Diversifying in-context links selection} (Appendix~\ref{app:diverse}): We explore how varying the selection of in-context links influences \our's LP performance. We find that \our exhibits varying degrees of robustness across different datasets. \textbf{Adjusting positive-to-negative in-context link ratios} (Appendix~\ref{app:ratio}): Instead of employing a balanced ratio of positive and negative in-context links during testing, we experiment with different ratios, including sets composed entirely of positive/negative samples. Surprisingly, we observe exclusive negative in-context links can achieve comparable performance to balanced sets on many datasets.

==> body/intro.tex <==
\section{Introduction}

Graph-structured data is ubiquitous across diverse domains, including social networks~\cite{liben-nowell_link_2003}, protein-protein interactions~\cite{szklarczyk_string_2019}, movie recommendations~\cite{koren_matrix_2009}, and citation networks~\cite{yang_revisiting_2016}. It encapsulates the complex relationships among entities, serving as a powerful data structure for analytical exploration. At the heart of graph analysis lies the task of link prediction (LP)~\cite{yang_evaluating_2015,dong_fakeedge_2022}, a crucial problem aimed at forecasting missing or future connections within these networks. Over the years, the quest to enhance LP accuracy has advanced the development of numerous methodologies~\cite{kumar_link_2020}, especially those based on Graph Neural Networks (GNNs)~\cite{kipf_semi-supervised_2017,hamilton_inductive_2018,xu_how_2018}.

Graph Neural Networks for Link Prediction~(GNN4LP) are a type of parametric link predictor, which can automatically learn the connectivity patterns by fitting the LP models to the target graphs. Typically, they are empowered with the most expressive capability~\cite{zhang_labeling_2021}, which makes them able to encode invariant link representations if and only if the links are symmetric with a permutation equivalence. The provable theoretical guarantee on their expressiveness makes them able to capture all possible link features. Equipped with such expressiveness, GNN4LP models are then supervised trained~\cite{zhang_link_2018} on the target graph to actively adapt to a certain connectivity pattern on the specific graph. However, their dependency on extensive training for each new graph dataset and the necessity for hyperparameter optimization~\cite{chamberlain_graph_2022,wang_neural_2023,dong_pure_2023} present notable challenges for their application across diverse graph environments. 

One type of LP methods, which is widely applied to different graphs without specific adjustments, is the traditional heuristics. By discovering and abstracting the universal structural properties underlying different graphs~\cite{barabasi_emergence_1999,watts_collective_1998,holland_stochastic_1983}, heuristics methods are developed based on observing the connectivity patterns existing in real-world graph datasets. For example, Common Neighbor~\cite{liben-nowell_link_2003}, the most famous one of heuristics, assumes the tendency of triadic closure~\cite{easley_networks_2010}, such that a friend's friend is likely to be friends in a social network. Nevertheless, these methods are not as expressive as the GNN4LPs, sacrificing their capability of capturing diverse structural features for the sake of better generalizability.

One immediate question is whether there is one singular LP model that can be seamlessly applied to any graph without expensive and specific tuning process.


% However, this approach relies on predefined heuristics, crafted from human expertise into the graph connectivity. Despite the initial success via capturing one specific connectivity pattern, they fail to capture all the effective structural features in the link prediction, leading to suboptimal link prediction performance when applied indiscriminately.
% However, this approach's reliance on predefined heuristics, crafted from human expertise into graph connectivity, may limit its adaptability to graphs with unique connectivity patterns, potentially leading to suboptimal link prediction performance when applied indiscriminately.

% \mao{Graph Neural Networks for Link Prediction~(GNN4LP) are then proposed to enable the model to capture more diverse structural patterns. Typically, the GNN4LP models can achieve the most-expressive structural pattern~\cite{zhang_labeling_2021}, i.e., the link representation should be invariant if and only if links are symmetric with a permutation equivalence, with provable theoretical guarantee on capturing all the possible effective patterns. Equipped with such expressiveness, GNN4LP models are then supervisely (add citation) trained on one specific graph to distuiguish the effective pattern on the specific graph. However, such training process requires extensive training for each new graph dataset and the necessity for hyperparameter optimization~\cite{chamberlain_graph_2022,wang_neural_2023,dong_pure_2023} present notable challenges for their application across diverse graph environments. One immediate question is whether a better to enjoy the benefit of expressiveness of the GNN4LP model without expensive and specific tuning process on each graph.}

% The other line of works is parametric link predictors, which automatically learn the connectivity patterns by fitting the LP models to the target graphs. These parametric methods, especially those Graph Neural Networks~\cite{kipf_semi-supervised_2017,hamilton_inductive_2018} for Link Prediction~(GNN4LP), have dominated the leaderboard of the link prediction tasks~\cite{hu_open_2021}. Typically, these GNN4LP are provably the most expressive models such that the link representation is permutation-invariant~\cite{zhang_labeling_2021}. They can capture more effective structural features compared to the simpler heuristics counterparts. However, their dependency on extensive training for each new graph dataset and the necessity for hyperparameter optimization~\cite{chamberlain_graph_2022,wang_neural_2023,dong_pure_2023} present notable challenges for their application across diverse graph environments.

 % with significantly better expressiveness and performance compared to the simpler heuristics counterparts.
% Nevertheless, such a performance boost comes with a price. These LP models have to be trained completely from scratch to fit the data whenever applied to any graph dataset. For example, the link prediction models trained on Facebook social networks cannot be directly applied to other graphs like citation networks. Moreover, to reach the optimal performance on any specific graph dataset, these models often have to undergo an extensive hyperparameter tuning process~\cite{chamberlain_graph_2022,wang_neural_2023,dong_pure_2023}. This process can impede the smooth application of LP methods on new graph datasets. 

Given that (1) the heuristics methods can be readily applied to any graphs without training based on common connectivity patterns and (2) the parametric model can automatically capture the connectivity patterns by fitting on the graph, a natural question arises:
\begin{center}
    \textbf{\textit{Can a singular LP model automatically learn and apply the connectivity pattern across new, unseen graphs without the need for direct training?}}
\end{center}
An affirmative response would not only pioneer a new frontier in graph machine learning but also align with the transformative potential observed in foundation models across text and image processing fields~\cite{brown_language_2020,kirillov_segment_2023}. These models' exceptional generalizability, driven by their capability of transfer learning~\cite{yosinski_how_2014}, offers a blueprint for the development of a universal LP model capable of broad applicability without explicit fitting.

% Foundation models have shown superior capability of generalization and can perform tasks on data from various domains. The success of its generalizability has been largely attributed to its capability of transfer learning~\cite{yosinski_how_2014}. Specifically, these models have been trained on a large scale of available data, which enables them to adapt the common knowledge learned during pretraining to new unseen datasets~\cite{bommasani_opportunities_2021}. Following the success of their great generalizability, we explore how to pretrain an LP model on a diverse set of graph datasets such that it can also be readily applied to any new unseen dataset without explicitly fitting.


\paragraph{Present work.} In this study, we introduce \maomask{I do not quite understand what is the universal link predictor}the Universal Link Predictor (\our), a novel model designed for immediate application across diverse graph environments\footnote{In this study, we focus on non-attributed graphs. This choice is informed by previous findings indicating that node attributes have minimal impact on the effectiveness of LP tasks~\cite{dong_pure_2023}. \maomask{I think another thing is that the feature can be hardly transferable. It may be a good choice to add one specific feature channel for each downstream task. Nonetheless, such specific rather than transferability is not the focus of our current paper}} without the prerequisite of model fitting. Our investigation starts by assessing whether existing LP models possess the capability to transfer connectivity pattern knowledge from one graph to another. \maomask{I think it could be better to say how we specilize the most-expressive structural representation for the given downstream task. That means, we know all the patterns from GNN, what pattern to utilize is specific on each dataset and selected by the ICL.} Through empirical and theoretical analyses spanning both heuristic and parametric link predictors, we uncover a significant challenge: negative transfer~\cite{wang_afec_2021} can happen when directly transferring the connectivity patterns across distinct graph datasets, including both real-world and synthetic examples. This complexity arises from the inherent diversity and flexibility of graph data distributions, leading to unique connectivity patterns for each graph.

To equip \our with the capability to adapt to diverse graphs without the need for training, we are inspired by the concept of in-context learning (ICL) as utilized by large language models (LLMs)~\cite{brown_language_2020}. ICL enables models to adapt to new datasets or tasks through the relevant demonstration examples~\cite{wang_label_2023}. Analogously, for adapting our LP model to a particular graph, we select a collection of in-context links to act as such demonstration examples. These in-context links not only provide a context for link prediction but also aid in capturing the unique connectivity pattern inherent to the graph in question. To achieve link representations that are inherently conditioned on the graph’s specific connectivity pattern, we employ an attention mechanism~\cite{vaswani_attention_2017,brody_how_2022}. This mechanism facilitates dynamic adjustment of link representations in response to the graph context, enabling the model to accurately reflect the unique connectivity patterns of each graph.

We have curated a diverse collection of graph datasets spanning multiple domains, providing a rich variety of connectivity patterns for benchmarking. Through extensive experiments on these datasets, we demonstrate the seamless applicability of \our to novel and unseen graph datasets without requiring dataset-specific fitting. Notably, \our, empowered with ICL, exhibits the capability to meet or even exceed the performance levels of LP models that have been pretrained and finetuned for specific target graphs. This achievement underscores \our's broad applicability and robust adaptability, establishing a groundbreaking approach to link prediction tasks.

In summary, our contributions to the field of link prediction are:
\begin{itemize}
\item We pioneer in highlighting the challenges of applying a singular LP model across various graph datasets due to conflicting connectivity patterns, a finding supported by both empirical evidence and theoretical analysis.
\item Addressing these challenges, we introduce \our, a novel LP approach leveraging ICL for dynamic adaptation to new graphs in real-time, thereby eliminating the need for traditional training processes.
\item The diverse collection of graph datasets we've collected facilitates extensive validation of \our's adaptability. Our experiments confirm that \our is not only capable of adjusting to any new graph dataset during inference but also achieves competitive performance, marking a significant advancement in link prediction methodologies.
\end{itemize}


==> body/tmp.tex <==
1. ICL: skill learning (flip labels) >  skill reconigtion

2. ICL: key link factor (CN, SP) motif 

3. Label Words are Anchors: An Information Flow Perspective for Understanding In-Context Learning

logisitc regression

foundational: LSP, GSP, FP


ICL: specification



Uncertainty can be found on the human-defined graph construction criteria~\cite{brugere2018network}. 
For instance, the construction knowledge relying on expert knowledge may lead to uncertainty in edges~\cite{ye2022generative}. 
\citet{Chen2023ExploringTP, li2023graphcleaner} observe that the mislabeled samples widely exist across datasets, where the popular \textsc{CiteSeer} dataset has more than 15\% mislabeling ratio. 
Despite the above uncertainty, different graph constructions with manual design can follow opposite principles. 
For instance, \arxiv~\cite{hu2020openOGB} and \arxivyear~\cite{lim2021largeLINKX} are two node classification datasets with identical graph information. 
The only difference lies in the label where \arxiv employs paper categories, and \arxivyear uses publication years as labels, resulting in conflicting homophily and heterophily properties~\cite{mao2023demystifyingNC}.
Therefore, when uncertainties and opposite graph constructions exist, the scaling behavior may not happen as the data does not obey the graph transferable principles. 


